On-line Non-Convex Constrained Optimization

Time-varying non-convex continuous-valued non-linear constrained optimization is a fundamental problem. We study conditions wherein a momentum-like regularising term allow for the tracking of local optima by considering an ordinary differential equation (ODE). We then derive an efficient algorithm based on a predictor-corrector method, to track the ODE solution.

==> analysis.tex <==
\section{An Analysis}
\label{sec:anal}


Let us consider the same assumptions as in Fattahi et al., \cite{fattahi2019}: 

	\begin{assumption}[Uniform Boundedness of Fattahi et al., \cite{fattahi2019}]\label{assum11}
		There exist constants $R_1>0$ and $R_2>0$ such that, for any discrete local trajectory $x_0,x_1,x_2,\hdots$, $\|x_k\|$ and the objective function of~\eqref{obj_reg} at $x_k$ are upper bounded by $R_1$ and $R_2$, respectively, for every $k=0,1,2,\hdots$.
	\end{assumption}

	\begin{assumption}[Non-singularity of Fattahi et al., \cite{fattahi2019}]\label{assum22}
		There exists a constant $c>0$ such that, for any discrete local trajectory $x_0,x_1,x_2,\hdots$, it holds that $\sigma_{\min}(\mathcal{J}(x_k))\geqslant c, ~k=0,1,2,\hdots$ where $\sigma_{\min}$ denotes the minimal singular value.
	\end{assumption}


Then, we can prove a similar structural result: 

	\begin{theorem}\label{thm:exist_unique} Let Assumption \ref{assum11} and Assumption \ref{assum22} hold. If the initial condition of~\eqref{eq:odeineq} is a local solution to the time-varying optimization at $t = 0$, then there exists a (unique) continuously differentiable solution $x:[0,T]\to\mathbb{R}^n$.
	\end{theorem}


We can derive a variety of negative results using \cite{ANDERSON2013}

==> inequalities.tex <==
The original optimisation program \cite{fattahi2019} would only account for equality constraints, being posed as,
\begin{align}
	\inf_{x\in \mathbb{R}^n} &  ~ f(x,t)\\ \text{ s.t. } & h_i(x) = d_i(t), \quad i = 1,\hdots,p
	\label{eq:originalproblem}
\end{align}
	
However, we can extend the analysis to inequality constraints thanks to a classical rewriting, \cite{Bertsekas/99}. Consider the following optimisation program containing inequalities,
\begin{align}
	\inf_{x\in \mathbb{R}^n} &  ~ f(x,t)\\ \text{ s.t. } & h_i(x) = d_i(t), \quad i = 1,\hdots,p \\
	& g_j(x) \leq e_j(t), \quad j = 1,\hdots,q
	\label{eq:inequalityproblem}
\end{align}
and its counterpart where new variables have been introduced to only have equality constraints, more amenable for us,
\begin{align}
	\inf_{x\in \mathbb{R}^n, \ z \in \mathbb{R}^p} &  ~ f(x,t)\\ \text{ s.t. } & h_i(x) = d_i(t), \quad i = 1,\hdots,p \\
	& g_j(x) + z_j^2 = e_j(t), \quad j = 1,\hdots,q
	\label{eq:equalityproblem}
\end{align}

Let $x \in \mathbb{R}^n$, then $x$ is a solution of \eqref{eq:inequalityproblem} if and only if there exists $z \in \mathbb{R}^p$ such that $[x~z]^\top$ is a solution of \eqref{eq:equalityproblem}. As a result, we can in a first time apply theorems to the equality program \eqref{eq:equalityproblem}, by considering the `inequality' ODE,
	\begin{align}
	%\boxed{
		\dot{X} = -\frac{1}{\alpha} \eta(X,t) + \theta(X)\dot{d}%}
	\tag{ODE$\geq$}\label{eq:odeineq}
	\end{align}
	where $X = [x~z]^\top$, $H = [h~g]^\top$,
	\begin{align}
	\eta(X,t) := & ~~ \left[I-\mathcal{J}_H(X)^\top(\mathcal{J}_H(X)\mathcal{J}_H(X)^\top)^{-1}\mathcal{J}_H(X)\right]\nabla_X f(x,t), \\
	\theta(X) ~ := & ~~ \mathcal{J}_H(X)^\top(\mathcal{J}_H(X)\mathcal{J}_H(X)^\top)^{-1}.
	\end{align}
	and $\mathcal{J}_H(X)$ is the Jacobian of the left hand side of the constraints.
	
Theorem 1 guarantees existence and uniqueness of a solution, after verifying assumptions 1,2, and assuming $X_0$ is a solution of the program \eqref{eq:equalityproblem} at time $t=0$. Theorem 2 further proves that any sequence of discrete local trajectories $(X^{\Delta t})$ for which $\Delta t \to 0$, converges to the solution $X$.
\begin{equation}
\lim_{\Delta t \to 0} \max_{0 \leq k \leq \lceil \nicefrac{T}{\Delta t} \rceil} \| X_k^{\Delta t} - X(t_k) \| = 0.
\end{equation}



%that there exists $\bar{t} >0$ such that for any $\bar{t} \geq \Delta t > 0$, we dispose of an AKKT tuple $\{x_k,z_k\}_{k=0}^{\lceil \frac{T}{\Delta t} \rceil$

==> problem_statement.tex <==
	\section{The Approach Formalised}
	\label{sec:problem_statement}

Let us consider the approach more formally:
	
	\begin{definition}[Based on Fattahi et al., \cite{fattahi2019}]
		\label{def:discrete}
		Given evenly spaced-out time steps $0 = t_0 < t_1 < t_2 < \hdots < t_N = T$ for some integer $N$, a sequence $x_0,x_1,x_2, \hdots, x_N$ is said to be a \emph{discrete local trajectory} of the time-varying optimization \eqref{eq:problem} if the following holds: 
		\begin{enumerate}
			\item $x_0$ is a local solution to the time-varying optimization \eqref{eq:problem} at time $t_0=0$;
			\item for $k=0,1,2, \hdots,N-1$, $x_{k+1}$ is local solution to
			\begin{align}
			\begin{array}{ll}
			\inf_{x\in \mathbb{R}^n} & f(x,t_{k+1}) ~+~  \alpha ~\frac{\|x - x_k\|^2}{2(t_{k+1}-t_k)} \label{obj_reg}\\[.3cm]
			\text{s.t.} & %h_i(x) = d_i(t_{k+1}) ~,~~~ i = 1,\hdots,m,
		h_i(x) = d_i(t_{k+1}), \quad i = 1,\hdots,p \\
	& g_j(x) \ge d_j(t_{k+1}),\quad j = 1,\hdots,q 	\end{array}
			\end{align}
			wherein $\| \cdot \|$ denotes the Euclidean norm.
		\end{enumerate}
	\end{definition}

%We relate such discrete local trajectories to the ODE:
%	\begin{align}
	%\boxed{
%		\dot{x} = -\frac{1}{\alpha} \eta(x,t) + \theta(x)\dot{d}%}
%	\tag{ODE}\label{eq:ode}
%	\end{align}
%	where
%	\begin{align}
%	\eta(x,t) := & ~~ \left[I-\mathcal{J}_h(x)^\top(\mathcal{J}_h(x)\mathcal{J}_h(x)^\top)^{-1}\mathcal{J}_h(x)\right]\nabla_x f(x,t), \\
%	\theta(x) ~ := & ~~ \mathcal{J}_h(x)^\top(\mathcal{J}_h(x)\mathcal{J}_h(x)^\top)^{-1}.
%	\end{align}
%	and $\mathcal{J}_h(x)$ is the Jacobian of the left hand side of the constraints. 



	\begin{definition}[Based on Fattahi et al., \cite{fattahi2019}]
		\label{def:continous}
		A continuously differentiable function $x: [0,T] \longrightarrow \mathbb{R}^n$ is said to be a \emph{continuous local trajectory} of the time-varying optimization \eqref{eq:problem} if the following holds:
		\begin{enumerate}
			\item $x(0)$ is a local solution to the time-varying optimization \eqref{eq:problem} at time $t=0$;
			\item $x$ is a solution to the ordinary differential equation \eqref{eq:odeineq}.
		\end{enumerate}
	\end{definition}
	
	\begin{definition}[Based on Fattahi et al., \cite{fattahi2019}]
		\label{def:spurious}
		A continuous local trajectory $x: [0,T] \longrightarrow \mathbb{R}^n$ is said to be a \emph{spurious local trajectory} 
		if its final state $x(T)$ does not belong to the region of attraction of a global solution to the time-varying optimization 
		\eqref{eq:problem} at time $t=T$. In other words, the trajectory is non-spurious if the initial value problem
		\begin{equation}
		\left\{
		\begin{array}{lcl}
		\dot{\bar{x}} & = & -\frac{1}{\alpha} \eta(\bar{x},T), \\[.2cm]
		\bar{x}(0) & = & x(T).
		\end{array}
		\right.
		\end{equation}
		admits a continuously differentiable solution $\bar{x}: \mathbb{R}_+ \longrightarrow \mathbb{R}^n$ such that $\bar{x}(t)$ converges 
		towards a global solution as $t \longrightarrow +\infty$.
	\end{definition}
